The Diagonal Problem for Higher-Order Recursion Schemes is Decidable

A non-deterministic recursion scheme recognizes a language of finite trees. This very expressive model can simulate, among others, higher-order pushdown automata with collapse. We show decidability of the diagonal problem for schemes. This result has several interesting consequences. In particular, it gives an algorithm that computes the downward closure of languages of words recognized by schemes. In turn, this has immediate application to separability problems and reachability analysis of concurrent systems.

==> strategy.tex <==

\section{Strategy}

For a HORS $\Ss$ and a set of symbols $\Sigma$, let $\Unb_\Sigma(\Ss)$ denote the property that holds if for every $n\in\Nat$ there is a tree generated by $\Ss$ in which every symbol from $\Sigma$ appears at least $n$ times. %labels at least $n$ nodes.
We want to give an algorithm deciding whether $\Unb_\Sigma(\Ss)$ for a given $\Sigma$ and $\Ss$.
When $\Ss$ is of order $0$, it is just (almost) a finite tree automaton, and thus deciding whether $\Unb_\Sigma(\Ss)$ holds in this case is easy.
For HORSes of higher order we repeatedly perform a transformation that decreases the order by one, finally reducing the situation to the easy case of order $0$.
This decreasing of order is done in two steps.
First, we ensure that the HORS is narrow: we create a HORS $\Ss'$ that is narrow, of the same order as $\Ss$, and such that $\Unb_\Sigma(\Ss)$ holds if and only if $\Unb_{\Sigma'}(\Ss')$ holds.
%In the second step we apply an appropriate normalization to the HORS, without changing the set of generated trees.
Then, in the narrow HORS $\Ss'$ we lower the order by one: 
we create a HORS $\Ss''$ that is of order smaller by one than $\Ss'$ (but is no longer narrow), and such that $\Unb_{\Sigma'}(\Ss')$ holds if and only if $\Unb_{\Sigma''}(\Ss'')$ holds.
The two steps are described in the next two sections.

